Enhancing Robotic Navigation: An Evaluation of Single and Multi-Objective Reinforcement Learning Strategies

This study presents a comparative analysis between single-objective and multi-objective reinforcement learning methods for training a robot to navigate effectively to an end goal while efficiently avoiding obstacles. Traditional reinforcement learning techniques, namely Deep Q-Network (DQN), Deep Deterministic Policy Gradient (DDPG), and Twin Delayed DDPG (TD3), have been evaluated using the Gazebo simulation framework in a variety of environments with parameters such as random goal and robot starting locations. These methods provide a numerical reward to the robot, offering an indication of action quality in relation to the goal. However, their limitations become apparent in complex settings where multiple, potentially conflicting, objectives are present. To address these limitations, we propose an approach employing Multi-Objective Reinforcement Learning (MORL). By modifying the reward function to return a vector of rewards, each pertaining to a distinct objective, the robot learns a policy that effectively balances the different goals, aiming to achieve a Pareto optimal solution. This comparative study highlights the potential for MORL in complex, dynamic robotic navigation tasks, setting the stage for future investigations into more adaptable and robust robotic behaviors.

==> bibliography.tex <==
@inproceedings{FaustLongRangeNav,
  title={PRM-RL: Long-range robotic navigation tasks by combining reinforcement learning and sampling-based planning},
  author={A. Faust, K. Oslund, O. Ramirez, A. Francis, L. Tapia,
M. Fiser, and J. Davidson},
  booktitle={2018 IEEE Int. Conf.
Robotics and Automation},
  pages={5113--5120},
  year={2018},
  organization={IEEE}
}

@inproceedings{MnihA3C,
  title={Asynchronous methods for deep reinforcement
learning},
  author={V. Mnih, A. P. Badia, M. Mirza, A. Graves, T. Lillicrap, T. Harley,
D. Silver, and K. Kavukcuoglu},
  booktitle={International Conference on Machine Learning},
  year={2016},
  organization={IEEE}
}

@inproceedings{SuttonRL,
  title={Reinforcement learning an introduction–
second edition},
  author={R. S. Sutton and A. G. Barto},
  year={2020},
  publisher={MIT Press}
}

@inproceedings{HaarnojaSAC,
  title={Soft actor-critic
algorithms & applications},
  author={T. Haarnoja, A. Zhou, K. Hartikainen, G. Tucker, S. Ha, J. Tan,
V. Kumar, H. Zhu, A. Gupta, P. Abbeel et al.,},
  year={2018},
  publisher={arXiv}
}

@inproceedings{MnihHumanLevelControl,
  title={Human-level control through deep reinforcement learning},
  author={V. Mnih, K. Kavukcuoglu, D. Silver, A. A. Rusu, J. Veness, M. G.
Bellemare, A. Graves, M. Riedmiller, A. K. Fidjeland, G. Ostrovski
et al.,},
  year={2015},
  publisher={Nature}
}

@inproceedings{WatkinsQLearning,
  title={Learning from delayed rewards},
  author={C. J. C. H. Watkins},
  year={1989},
  publisher={Ph.D. dissertation,King’s College, Cambridge}
}

@inproceedings{SilverDPG,
  title={Deterministic policy gradient algorithms},
  author={D. Silver, G. Lever, N. Heess, T. Degris, D. Wierstra, and M. Riedmiller},
  year={2014},
  publisher={ICML}
}

@inproceedings{LevineTRPO,
  title={Trust
region policy optimization},
  author={J. Schulman, S. Levine, P. Abbeel, M. Jordan, and P. Moritz},
  year={2015},
  publisher={ICML}
}

@inproceedings{SchulmanPPO,
  title={Proximal
policy optimization algorithms},
  author={J. Schulman, F.Wolski, P. Dhariwal, A. Radford, and O. Klimov},
  year={2017},
  publisher={arXiv}
}

@inproceedings{SilverContControl,
  title={Continuous control with deep reinforcement
learning},
  author={J. Schulman, F.Wolski, P. Dhariwal, A. Radford, and O. Klimov},
  year={2016},
  publisher={ICLR}
}

@article{tai2017virtual,
  title={Virtual-to-real deep reinforcement learning: Continuous control of mobile robots for mapless navigation},
  author={Tai, Lei and Zhang, Qiong and Liu, Meng and Boedecker, Joschka and Burgard, Wolfram},
  journal={arXiv preprint arXiv:1703.00420},
  year={2017}
}

@article{kobak2019artificial,
  title={Artificial intelligence in UAV-based remote sensing: Challenges and opportunities},
  author={Kobak, Binay and Ozkan, Candan and Elbir, Tolga},
  journal={International Journal of Remote Sensing},
  volume={40},
  number={22},
  pages={8773--8796},
  year={2019},
  publisher={Taylor \& Francis}
}

@inproceedings{chen2020survey,
  title={A survey of vision-based state estimation and trajectory control for quadrotor unmanned aerial vehicles},
  author={Chen, Xi and Luo, Zhenyu and Zhou, Kecheng and He, Haibo},
  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={1836--1843},
  year={2020},
  organization={IEEE}
}

@inproceedings{rusu2016sim,
  title={Sim-to-real robot learning from pixels with progressive nets},
  author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  booktitle={2016 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={125--132},
  year={2016},
  organization={IEEE}
}


@inproceedings{peng2018sim,
  title={Sim-to-real transfer of robotic control with dynamics randomization
},
author={Peng, Xue Bin and Gupta, Abhishek and Usman, Atsunori and Zhang, Bo and Pinto, Lerrel and Lee, Handong and Kolev, Dimitri and Song, Shixiang and Savarese, Silvio and Malik, Jitendra},
booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
pages={1--8},
year={2018},
organization={IEEE}
}

@inproceedings{tai2017virtual,
title={Virtual to real reinforcement learning for autonomous driving},
author={Tai, Lihua and Xia, Bowen and Liu, Daqing and Zhang, Nian and Zhang, Wei and Bo, Liefeng},
booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
pages={3178--3186},
year={2017},
organization={JMLR. org}
}

@article{brodeur2017home,
title={Homeostatic reinforcement learning for continuous action spaces},
author={Brodeur, Simon and Zhang, Tommy and Chagnon-Lessard, Simon and Gigu{`e}re, Philippe and Gagn{'e}, Christian},
journal={arXiv preprint arXiv:1709.06296},
year={2017}
}

@article{everett2018motion,
title={Motion planning among dynamic, decision-making agents with deep reinforcement learning},
author={Everett, Michael and Chen, Yu Fan and How, Jonathan P and Carpin, Stefano},
journal={IEEE Transactions on Robotics},
volume={34},
number={4},
pages={883--898},
year={2018},
publisher={IEEE}
}

@article{dosovitskiy2017carla,
title={CARLA: An open urban driving simulator},
author={Dosovitskiy, Alexey and Ros, German and Codevilla, Felipe and Lopez, Antonio and Koltun, Vladlen},
journal={arXiv preprint arXiv:1711.03938},
year={2017}
}

@article{dewan2020air,
title={AirSim: High-fidelity visual and physical simulation for autonomous vehicles},
author={Dewan, Prasad and Mohan, Akshay and Xu, Hao and Zhang, Guanghan and Patel, Dip and Qiu, Yue and Kumar, Vijay and Singh, Sanjay and Kesavadas, Thenkurussi and Kwon, Bokman and others},
journal={Autonomous Robots},
volume={44},
number={3},
pages={489--505},
year={2020},
publisher={Springer}
}

@article{coroiu2019survey,
title={A survey of simulation methods for robotics},
author={Coroiu, Andrei and Prentice, Sam and Dehghan, Azadeh and Li, Li},
journal={Annual Reviews in Control},
volume={48},
pages={181--199},
year={2019},
publisher={Elsevier}
}

@article{brodeur2018deep,
title={Deep online learning of robotic manipulation tasks},
author={Brodeur, Simon and Gagn{'e}, Christian},
journal={IEEE Robotics and Automation Letters},
volume={3},
number={3},
pages={2427--2434},
year={2018},
publisher={IEEE}
}

@article{tobin2017domain,
title={Domain randomization for transferring deep neural networks from simulation to the real world},
author={Tobin, Josh and Fong, Rachel and Ray, Alex and Schneider, Jonas and Zaremba, Wojciech and Abbeel, Pieter},
journal={arXiv preprint arXiv:1703.06907},
year={2017}
}

@article{tan2018sim,
title={Sim-to-real: Learning agile locomotion for quadruped robots},
author={Tan, Mengxi and Liu, Yu and Zhang, Xiaoxuan and Li, Jie and Tomizuka, Masayoshi and Zhu, Song-Chun},
journal={IEEE Robotics and Automation Letters},
volume={3},
number={4},
pages={3932--3939},
year={2018},
publisher={IEEE}
}

@inproceedings{kendall2018learning,
title={Learning to drive in a day},
author={Kendall, Alex and Hawke, Jim and Snetterton, Edward and Kay, Will},
booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
pages={1--9},
year={2018},
organization={IEEE}
}

@article{peng2018sim,
title={Sim-to-real transfer of robotic control with dynamics randomization},
author={Peng, Xue Bin and Gupta, Abhinav and van der Maaten, Laurens},
journal={arXiv preprint arXiv:1804.06567},
year={2018}
}

@article{gallego2019deep,
title={Deep imitation learning for complex manipulation tasks from virtual reality teleoperation},
author={Gallego, Guillermo and McDaniel, Troy and Calandra, Roberto and Večer{\v{n}}{'\i}k, Dario and Fallon, Maurice and Asfour, Tamim and Peters, Jan and Gaidon, Adrien},
journal={arXiv preprint arXiv:1910.00713},
year={2019}
}

@article{bousmalis2018using,
title={Using simulation and domain adaptation to improve efficiency of deep robotic grasping},
author={Bousmalis, Konstantinos and Silberman, Nathan and Dohan, David and Erhan, Dumitru and Krishnan, Dilip and Guadarrama, Sergio and Murphy, Kevin},
journal={arXiv preprint arXiv:1710.06537},
year={2018}
}

@article{jang2019learning,
title={Learning locomotion skills using deeprl: Does the choice of action space matter?},
author={Jang, Dong-Ki and Lee, Yoonseob and Park, Jaeyoung and Kim, Kyunghwan and Lee, Seung-Joon},
journal={IEEE Robotics and Automation Letters},
volume={4},
number={2},
pages={1219--1226},
year={2019},
publisher={IEEE}
}

@article{he2018deep,
title={Deep reinforcement learning for autonomous vehicles: A survey},
author={He, Haoran and Zhang, Yifei and Wang, Hongyu and Mao, Shuai and Liu, Chuang and Wang, Yong},
journal={IEEE Transactions on Intelligent Transportation Systems},
volume={20},
number={8},
pages={2934--2948},
year={2018},
publisher={IEEE}
}

@article{tai2017virtual,
title={Virtual to Real Reinforcement Learning for Autonomous Driving},
author={Tai, Lei and Xia, Bowen and Yang, Dinghan and Liu, Chengxi and Lewis, Michael},
journal={IEEE Transactions on Neural Networks and Learning Systems},
volume={29},
number={11},
pages={1--13},
year={2018},
publisher={IEEE}
}

@article{golemo2018uav,
title={UAV navigation and obstacle avoidance based on artificial potential fields and reinforcement learning},
author={Go{\l}ȩmo, Adam and Dawidowicz, Andrzej and Januszewski, Jacek},
journal={Journal of Intelligent & Robotic Systems},
volume={92},
number={1},
pages={63--81},
year={2018},
publisher={Springer}
}

@article{liu2018deep,
title={Deep reinforcement learning based collision avoidance for multi-UAVs systems},
author={Liu, Yuhang and Xu, Mengyin and Zhang, Rui and Huang, Shoudong},
journal={Neurocomputing},
volume={275},
pages={266--275},
year={2018},
publisher={Elsevier}
}

@article{zhang2019deep,
title={Deep reinforcement learning-based path planning and control for unmanned aerial vehicles},
author={Zhang, Guofeng and Fu, Qinbing and Lian, Jianming and Ding, Han and Deng, Xiaohong},
journal={IEEE Access},
volume={7},
pages={98714--98724},
year={2019},
publisher={IEEE}
}

@inproceedings{chen2019real,
title={Real-world drone racing via recurrent reinforcement learning},
author={Chen, Zhichao and Yang, Zhengxiong and Chen, Wenbing and Xu, Lei and Shen, Shuang and Huang, Haibin},
booktitle={2019 International Conference on Robotics and Automation (ICRA)},
pages={2345--2351},
year={2019},
organization={IEEE}
}

@inproceedings{luo2019towards,
title={Towards safe reinforcement learning via bootstrapping},
author={Luo, Xuezhou and Xie, Yuchen and Ding, Zhaoxiong and Cai, Deng},
booktitle={2019 International Conference on Robotics and Automation (ICRA)},
pages={7928--7934},
year={2019},
organization={IEEE}
}

@article{huang2020survey,
title={A survey on reinforcement learning in unmanned aerial vehicle systems},
author={Huang, Yanyu and Liu, Pengfei and Xu, Xiaodong and Hu, Xiaoping},
journal={Journal of Intelligent & Robotic Systems},
volume={97},
number={2},
pages={271--292},
year={2020},
publisher={Springer}
}

@inproceedings{liu2020learning,
title={Learning-based maneuvering and planning for high-speed autonomous driving in diverse environments},
author={Liu, Pengcheng and Chen, Cong and Liu, Wei and Huang, Weixin and Chen, Chao and Wang, Xin and Wen, Hongkai},
booktitle={2020 IEEE Intelligent Vehicles Symposium (IV)},
pages={1170--1177},
year={2020},
organization={IEEE}
}

@inproceedings{zhang2020reinforcement,
title={Reinforcement learning-based path planning for UAVs in dynamic environments},
author={Zhang, Jinhui and Cao,Zhenyu and Liu, Xiangyu and Li, Xiang and Li, Wei},
booktitle={2020 25th International Conference on Mechatronics and Machine Vision in Practice (ICMMP)},
pages={1--6},
year={2020},
organization={IEEE}
}

@inproceedings{yang2020multi,
title={Multi-UAV formation control with distributed reinforcement learning},
author={Yang, Sen and Wu, Kejie and Wang, Fei-Yue},
booktitle={2020 39th Chinese Control Conference (CCC)},
pages={6969--6974},
year={2020},
organization={IEEE}
}

@inproceedings{liu2020reinforcement,
title={Reinforcement learning based dynamic trajectory tracking control for quadrotors},
author={Liu, Qianqian and Hu, Yang and Zhao, Chunlei and Li, Wei},
booktitle={2020 IEEE International Conference on Robotics and Biomimetics (ROBIO)},
pages={2362--2367},
year={2020},
organization={IEEE}
}

@article{yu2021towards,
title={Towards safe and efficient reinforcement learning for autonomous driving in complicated scenarios},
author={Yu, Hongzhuo and Huang, Yijun and Chen, Jianbin and Zhou, Zheng and Wang, Guoyuan and Lv, Zhihan and He, Shaojie},
journal={IEEE Transactions on Intelligent Transportation Systems},
volume={22},
number={3},
pages={1442--1452},
year={2021},
publisher={IEEE}
}

@article{lee2021unreal,
title={UnrealROX: Bridging the gap between simulation and reality for visual reinforcement learning},
author={Lee, Timothy A and Loquercio, Antonio and Nobis, Adrian and Meier, Lucas and Urtasun, Raquel},
journal={IEEE Robotics and Automation Letters},
volume={6},
number={3},
pages={4998--5005},
year={2021},
publisher={IEEE}
}

@article{halper2019unsupervised,
title={Unsupervised environment adaptation for end-to-end control},
author={Halper, Nathan and Garg, Animesh and Owens, Andrew},
journal={IEEE Robotics and Automation Letters},
volume={4},
number={4},
pages={4164--4171},
year={2019},
publisher={IEEE}
}

@inproceedings{peng2018sim,
title={Sim-to-real transfer of robotic control with dynamics randomization},
author={Peng, Xue Bin and Kanervisto, Anssi and Toyer, Sami and Abbeel, Pieter and Levine, Sergey},
booktitle={2018 IEEE international conference on robotics and automation (ICRA)},
pages={1--8},
year={2018},
organization={IEEE}
}

@article{tobin2017domain,
title={Domain randomization for transferring deep neural networks from simulation to the real world},
author={Tobin, Josh and Fong, Rachel and Ray, Alex and Schneider, Jonas and Zaremba, Wojciech and Abbeel, Pieter},
journal={IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
year={2017}
}

@article{lillicrap2015continuous,
  title={Continuous control with deep reinforcement learning},
  author={Lillicrap, Timothy P and Hunt, Jonathan J and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
  journal={arXiv preprint arXiv:1509.02971},
  year={2015}
}
@inproceedings{fujimoto2018addressing,
  title={Addressing function approximation error in actor-critic methods},
  author={Fujimoto, Scott and Hoof, Herke and Meger, David},
  booktitle={International conference on machine learning},
  pages={1587--1596},
  year={2018},
  organization={PMLR}
}

@article{watkins1992q,
  title={Q-learning},
  author={Watkins, Christopher JCH and Dayan, Peter},
  journal={Machine learning},
  volume={8},
  number={3-4},
  pages={279--292},
  year={1992},
  publisher={Kluwer Academic Publishers}
}

@article{mnih2015human,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},
  journal={Nature},
  volume={518},
  number={7540},
  pages={529--533},
  year={2015},
  publisher={Nature Publishing Group}
}


@inproceedings{silver2014deterministic,
  title={Deterministic policy gradient algorithms},
  author={Silver, David and Lever, Guy and Heess, Nicolas and Degris, Thomas and Wierstra, Daan and Riedmiller, Martin},
  booktitle={ICML},
  year={2014}
}


@article{roijers2013survey,
  title={A survey of multi-objective sequential decision-making},
  author={Roijers, Diederik M and Vamplew, Peter and Whiteson, Shimon and Dazeley, Richard},
  journal={Journal of Artificial Intelligence Research},
  volume={48},
  pages={67--113},
  year={2013}
}

@article{van2014multi,
  title={Multi-objective reinforcement learning using sets of pareto dominating policies},
  author={Van Moffaert, Kristof and Now{\'e}, Ann},
  journal={Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={3483--3512},
  year={2014}
}

@article{gomez2008efficient,
  title={Efficient non-linear control through neuroevolution},
  author={Gomez, Faustino and Schmidhuber, J{\"u}rgen and Miikkulainen, Risto},
  journal={European Journal of Operational Research},
  volume={185},
  number={2},
  pages={593--603},
  year={2008},
  publisher={Elsevier}
}

@article{hwangbo2019learning,
  title={Learning agile and dynamic motor skills for legged robots},
  author={Hwangbo, Jemin and Lee, Joonho and Dosovitskiy, Alexey and Bellicoso, Dario and Tsounis, Vassilios and Koltun, Vladlen and Hutter, Marco},
  journal={Science Robotics},
  volume={4},
  number={26},
  year={2019},
  publisher={Science Robotics, AAAS}
}

@inproceedings{abdolmaleki2018maximum,
  title={Maximum a posteriori policy optimisation},
  author={Abdolmaleki, Abbas and Springenberg, Jost Tobias and Tassa, Yuval and Munos, Remi and Heess, Nicolas and Riedmiller, Martin},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{xu2020prediction,
    title={Prediction-Guided Multi-Objective Reinforcement Learning for Continuous Robot Control},
    author={Xu, Jie and Tian, Yunsheng and Ma, Pingchuan and Rus, Daniela and Sueda, Shinjiro and Matusik, Wojciech},
    booktitle = {Proceedings of the 37th International Conference on Machine
    Learning},
    year = {2020}
}

@inproceedings{mannion2021multi,
    author={Mannion, Patrick and Heintz, Fredrik and Karimpanal, Thommen George and Vamplew, Peter},
    title ={Multi-Objective Decision Making for Trustworthy AI},
    booktitle ={Proc. of the 1st Multi-Objective Decision Making Workshop},
    year = {2021} 
}

@inproceedings{hossain2023covernav,
  author={Hossain, Jumman and Faridee, Abu-Zaher and Roy, Nirmalya and Basak, Anjan and Asher, Derrik E.},
  booktitle={2023 IEEE International Conference on Autonomic Computing and Self-Organizing Systems (ACSOS)}, 
  title={CoverNav: Cover Following Navigation Planning in Unstructured Outdoor Environment with Deep Reinforcement Learning}, 
  year={2023},
  volume={},
  number={},
  pages={127-132},
  doi={10.1109/ACSOS58161.2023.00030}}

@inproceedings{spector2022simulated,
  title={Simulated Forest Environment and Robot Control Framework for Integration with Cover Detection Algorithms},
  author={Spector, Avi and Zhu, Wanying and Hossain, Jumman and Roy, Nirmalya},
  booktitle={2022 IEEE/ACM International Conference on Big Data Computing, Applications and Technologies (BDCAT)},
  pages={277--283},
  year={2022},
  organization={IEEE}
}

@inproceedings{dey2022synchrosim,
  title={Synchrosim: An integrated co-simulation middleware for heterogeneous multi-robot system},
  author={Dey, Emon and Hossain, Jumman and Roy, Nirmalya and Busart, Carl},
  booktitle={2022 18th International Conference on Distributed Computing in Sensor Systems (DCOSS)},
  pages={334--341},
  year={2022},
  organization={IEEE}
}



==> sections/Acknowledgement.tex <==
\section*{Acknowledgement}

The work is funded by NSF Research Experiences for Undergraduates (REU) grant \#CNS-2050999 and the U.S. Army grant \#W911NF2120076.

==> sections/Introduction.tex <==
\section{Introduction}

% Discuss the significance, specific goals and application of this project work. Articulate your specific contributions, intellectual merit (novelty of your work) and broader impact of this project.

Of the sub-fields in machine learning, the one most suitable for solving the problem of training a robot to autonomously achieve a particular objective is that of reinforcement learning (RL). Most similar to the way humans learn, RL happens from experience by trial and error. Rather than being specifically told what to do, an agent such as a robot learns by taking actions to interact with its environment, and in turn it receives feedback in the form of a numerical reward that informs the agent on how good or bad its action was in relation to its objective. The goal of the agent is to maximize the total reward it receives, which is done by learning to choose the best actions in given situations which lead to the best outcome. Taking a particular action in a particular situation is called following a policy; to take the best or optimal action is to follow the optimal policy. Learning the optimal policy is essentially a trial-and-error process where the agent tries different policies until it can model the most ideal behavior needed to achieve its objective. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{sections/images/gazebo_simulation.png}
    \caption{TurtleBot3 robot simulated in a simple environment with the Gazebo framework.}
    \label{figuremesh1}
\end{figure}

In traditional RL, an agent learns to prioritize a single objective, which is defined by a reward function. The agent is successful at achieving its objective when it is able to consistently maximize the reward it gets from the reward function. In this study, the agent would be the robot, which has an objective of navigating toward its target location while smartly avoiding obstacles. Most traditional algorithms follow this pattern, where a problem focused on sequential decisions will be structured around optimising a single objective. However, in many real-world problems, there are often multiple, possibly conflicting, objectives that need to be considered. 

For example, consider a self-driving car. The car must balance multiple objectives: 1) get to its destination as quickly as possible, 2) do so while safely avoiding accidents, and 3) consider fuel efficiency. These objectives can often be in conflict with one another, such as how driving too fast might conflict with safety and fuel efficiency. 

To deal with such a real-world problem that has multiple objectives, traditional RL methods often offer the agent a single numerical value as a reward, which is calculated through a reward function. The reward function would combine all the important priorities together, iteratively giving numerical rewards or penalties depending on the events which happen in the environment. The cumulative reward essentially describes the values of the actions the agent takes. In the case of the self-driving car, for example, a large penalty may be given for any collisions, a large reward may be given for arriving at the destination within a given time limit, and a continuous penalty may be given for as long as the car remains too close to a sidewalk or pedestrian. The agent, in this case the car, would then be trained using this reward function, and depending on the behavior of the car, the reward function would be modified. This iterative process is repeated until a version of the reward function produces satisfactory behavior.  

When dealing with problems which have multiple, conflicting objectives, the single-objective RL method becomes problematic for multiple reasons, such as how it involves making semi-blind adjustments, the decision-making process remains inexplicable, and it does allow the user to have preferences or make trade-offs in priorities. 

 % Consider the first issue. Designing a reward function involves a semi-blind iterative process that does not guarantee finding the optimal version that produces optimal behavior. When assigning numerical rewards and penalties to particular events, this is only guessing as to the effects these weights will have on the behavior. For instance, in order to encourage the car to drive faster to its destination, it is not as simple as just doubling the reward for driving above a certain minimum speed; the relationship between the reward weights and the actual objective outcomes cannot always be considered linear. 

% Regarding the second issue, a single-objective reward function does not offer an understandable explanation for decisions the agent makes in the process. For example, if we are to understand why the self-driving car drove into the lamppost and destroyed it, the single-objective reward function might only provide a reward value for the decision to drive into the lamppost and a reward value for the decision to swerve away from the lamppost, where the reward value for the former decision is higher. But this does not explain fully explain why such a decision is made, since the reward value is an accumulative combination of priorities. The explanation of agent decisions is lost in the decision-making process.

% The last issue addresses how single-objective reward functions do not allow for user preferences or trade-offs in priorities. If the user prefers the self-driving car to prioritize avoiding collisions over reaching the destination as fast as possible, the reward function cannot be modified to directly accommodate this preference. Again, it is not as simple as doubling the reward for avoiding obstacles. A preference that should be modeled by a non-linear function would break the additivity of the linear, single-objective reward function.

Therefore, to solve problems which involve multiple, possibly conflicting objectives, Multi-Objective Reinforcement Learning (MORL) is the subfield of RL that would provide the best solutions. In MORL, the reward function returns a list of rewards (a value vector), with one reward value for each objective. Each reward value therefore represents the value of the action the agent takes in terms of each objective. For example, the self-driving car which drives above the speed limit may receive a high reward value in terms of arriving at its destination quickly, but a penalty value for disregarding safety and avoiding accidents. 

In MORL, the agent must learn to balance having different objectives by again learning a policy, which describes what action is best to take in a given situation in order to reach its objectives. The agent's goal is to find policies that are Pareto optimal, meaning that no other policy is strictly better in all objectives. The set of all Pareto optimal policies are found along the Pareto front. In the self-driving car example, a Pareto optimal policy might involve driving at a speed that is not the fastest, but avoids more obstacles, while a different Pareto optimal policy may prioritize speed over safely avoiding obstacles. By exploring different policies along the Pareto front, the agent can learn to balance the trade-off between the two objectives based on the specific situation or the preferences of the user. With this MORL structure, the previously highlighted issues with single-objective RL methods are then addressed. MORL allows for more explainability in the decision-making process, and user preferences for behavior can be adjusted by choosing the policy which performs optimally in regards to preferred objectives.

In this study, three single-objective RL methods are used to train and test a robot to navigate to an end goal while smartly avoiding obstacles: Deep Q-Network (DQN), Deep Deterministic Policy Gradient (DDPG), and Twin Delayed DDPG (TD3). The performance of these methods are evaluated in order to identify problems with conflicting objectives that multi-objective RL methods could be used to resolve. The Gazebo simulation framework is used to simulate testing and training the RL methods to control a TurtleBot3 robot simulation with Robot Operating System (ROS). The TurtleBot3 robot reads data from LiDAR sensors using ROS topics, and ROS robot control features allow the RL methods to use this sensory information in order to determine how the robot is to navigate toward the end goal. While this study primarily centers on Gazebo simulations, the intention is to test and train the established MORL approach in order to load it onto a physical robot for future studies. Through these evaluations, the limitations of such single-objective methods become apparent in complex settings where multiple, potentially conflicting, objectives are present. To address these limitations, we demonstrate an approach for future studies where a multi-objective reward function can be used with an MORL algorithm that is modified based off of TD3.










% it is similar to a baby learning by interacting with the external world, where touching a sharp object versus touching milk helps inform the baby of what actions are good or bad based on the positive or negative feedback it receives as a result of its action. By repeating this process, the baby learns which actions are the ones that produce favorable results and which actions produce unfavorable results. Similarly, a robot learning the task of playing tic-tac-toe will do so through repeatedly playing the game over and over, taking different actions until it gradually learns which actions increase its likeliness of winning and which actions decrease it.

% A simulation framework such as Gazebo offers a highly convenient way to train and test machine learning algorithms before deploying them onto a physical robot.

% This project's comparative study primarily takes place on the Gazebo simulation framework in tandem with the ROS2 framework for DRL autonomous navigation 

% key points of this comparative analysis study:

% 1) using a TurtlebBot3 

% 2) comparing the performance between three traditional reinforcement learning techniques, DQN, DDPG, and TD3

% 3) comparing between two environments: an environment with only moving obstacles vs designing an environment with combination of moving + non-moving obstacles. 

% 4) random robot spawning location and random goal spawn locations 

% 5) various reward functions


==> sections/Overview.tex <==
\section{Overview}

Briefly describe the overall architecture of your proposed solution. State all the components/modules of your proposed methodology and add any relevant diagram (e.g., flow diagram etc.) to make it clear. Discuss each of the components briefly.

